UniRank: Unimodal Bandit Algorithm for Online Ranking

We tackle a new emerging problem, which is finding an optimal monopartite matching in a weighted graph. The semi-bandit version, where a full matching is sampled at each iteration, has been addressed by \cite{ADMA}, creating an algorithm with an expected regret matching $O(\frac{L\log(L)}{\Delta}\log(T))$ with $2L$ players, $T$ iterations and a minimum reward gap $\Delta$. We reduce this bound in two steps. First, as in \cite{GRAB} and \cite{UniRank} we use the unimodality property of the expected reward on the appropriate graph to design an algorithm with a regret in $O(L\frac{1}{\Delta}\log(T))$. Secondly, we show that by moving the focus towards the main question `\emph{Is user $i$ better than user $j$?}' this regret becomes $O(L\frac{\Delta}{\tilde{\Delta}^2}\log(T))$, where $\Tilde{\Delta} > \Delta$ derives from a better way of comparing users. Some experimental results finally show these theoretical results are corroborated in practice.

==> macros.tex <==
\definecolor{orange}{rgb}{1.0, 0.5, 0.0}
\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.2}

\newcommand{\commentelisa}[1]{{\color{red}Elisa: #1}}
%\newcommand{\commentcsg}[1]{{\color{darkgreen}Camille: #1}}
\newcommand{\writecsg}[1]{{\color{darkgreen}#1}}
\newcommand{\writerg}[1]{{\color{darkgreen}#1}}
\newcommand{\forlater}[1]{{\color{orange}Plus tard: #1}}

%\renewcommand{\commentrg}[1]{}
%\renewcommand{\commentelisa}[1]{}
%\renewcommand{\commentcsg}[1]{}
%\renewcommand{\writecsg}[1]{#1}
%\renewcommand{\writerg}[1]{#1}
\renewcommand{\forlater}[1]{}


\RequirePackage{amsthm}
%\newtheorem{definition}{Definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{assumption}{Assumption}
%\newtheorem*{assumption0}{Assumption 3.0}
%\newtheorem{illustration}{Illustration}
\newtheorem*{assumption0s}{Assumption 3.1$^*$}
%\newtheorem{remark}{Remark}

\newcommand{\ouralgo}{{UniRank}}
\newcommand{\ouralgolong}{{Unimodal Bandit Algorithm for Online Ranking}}
\newcommand{\ouralgobis}{{UniSRank}}
\newcommand{\ouralgobislong}{{Unimodal Bandit Algorithm for Online Strict Ranking}}

\newcommand{\ourmodel}{{MM}}
\newcommand{\ourstrictmodel}{{sMM}}

\newcommand{\mapping}{{\cal F}}
\newcommand{\GG}{{G_\text{rank}}}
\newcommand{\lGG}{{G_\text{lrank}}}


\newcommand{\muh}[1]{\sum_\ell\hat\rho_{#1_\ell,\ell}(t)}

\newcommand\nullCell{\cellcolor{black}}
\DeclareMathOperator*{\recommended}{Rec}


==> macros_math.tex <==
\RequirePackage{amsmath, amssymb, mathrsfs, bm, dsfont}

\newcommand{\vect}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\av}{\vect{a}}
\newcommand{\bv}{\vect{b}}
\newcommand{\cv}{\vect{c}}
\newcommand{\dv}{\vect{d}}
\newcommand{\ev}{\vect{e}}
\newcommand{\fv}{\vect{f}}
\newcommand{\gv}{\vect{g}}
\newcommand{\hv}{\vect{h}}
\newcommand{\iv}{\vect{i}}
\newcommand{\jv}{\vect{j}}
\newcommand{\kv}{\vect{k}}
\newcommand{\lv}{\vect{l}}
\newcommand{\mv}{\vect{m}}
\newcommand{\nv}{\vect{n}}
\newcommand{\ov}{\vect{o}}
\newcommand{\pv}{\vect{p}}
\newcommand{\qv}{\vect{q}}
\newcommand{\rv}{\vect{r}}
\newcommand{\sv}{\vect{s}}
\newcommand{\tv}{\vect{t}}
\newcommand{\uv}{\vect{u}}
\newcommand{\vv}{\vect{v}}
\newcommand{\wv}{\vect{w}}
\newcommand{\xv}{\vect{x}}
\newcommand{\yv}{\vect{y}}
\newcommand{\zv}{\vect{z}}
\newcommand{\ellv}{\vect{\ell}}

\newcommand{\onev}{{\pmb{1}}}
\newcommand{\alphav}{{\pmb{\alpha}}}
\newcommand{\betav}{{\pmb{\beta}}}
\newcommand{\gammav}{{\pmb{\gamma}}}
\newcommand{\kappav}{{\pmb{\kappa}}}
\newcommand{\muv}{{\pmb{\mu}}}
\newcommand{\omegav}{{\pmb{\omega}}}
\newcommand{\piv}{\vect{\pi}}
\newcommand{\rhov}{{\pmb{\rho}}}
\newcommand{\sigmav}{{\pmb{\sigma}}}
\newcommand{\tauv}{{\pmb{\tau}}}
\newcommand{\thetav}{{\pmb{\theta}}}
\newcommand{\xiv }{{\pmb{\xi}}}
\newcommand{\zetav}{{\pmb{\zeta}}}



\newcommand{\mat}[1]{{\pmb{#1}}} % vector in bold
\newcommand{\Am}{\mat{A}}
\newcommand{\Bm}{\mat{B}}
\newcommand{\Cm}{\mat{C}}
\newcommand{\Dm}{\mat{D}}
\newcommand{\Em}{\mat{E}}
\newcommand{\Fm}{\mat{F}}
\newcommand{\Gm}{\mat{G}}
\newcommand{\Hm}{\mat{H}}
\newcommand{\Imat}{\mat{I}}
\newcommand{\Jm}{\mat{J}}
\newcommand{\Km}{\mat{K}}
\newcommand{\Lm}{\mat{L}}
\newcommand{\Mm}{\mat{M}}
\newcommand{\Nm}{\mat{N}}
\newcommand{\Om}{\mat{O}}
\newcommand{\Pm}{\mat{P}}
\newcommand{\Qm}{\mat{Q}}
\newcommand{\Rm}{\mat{R}}
\newcommand{\Sm}{\mat{S}}
\newcommand{\Tm}{\mat{T}}
\newcommand{\Um}{\mat{U}}
\newcommand{\Vm}{\mat{V}}
\newcommand{\Wm}{\mat{W}}
\newcommand{\Xm}{\mat{X}}
\newcommand{\Ym}{\mat{Y}}
\newcommand{\Zm}{\mat{Z}}
\newcommand{\zerom}{\mat{0}}

\newcommand{\Deltam}{{\mbox{\boldmath$\Delta$}}}
\newcommand{\Gammam}{{\mbox{\boldmath$\Gamma$}}}
\newcommand{\Omegam}{{\mbox{\boldmath$\varOmega$}}}
\newcommand{\Lambdam}{{\mbox{\boldmath$\Lambda$}}}
\newcommand{\Sigmam}{{\mbox{\boldmath$\varSigma$}}}
\newcommand{\Phim}{{\mbox{\boldmath$\Phi$}}}
\newcommand{\Pim}{{\mbox{\boldmath$\Pi$}}}
\newcommand{\Thetam}{{\mbox{\boldmath$\varTheta$}}}




\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}

\newcommand{\RR}{\mathds{R}} %real numbers
\newcommand{\NN}{\mathds{N}} %natural numbers
\newcommand{\ZZ}{\mathds{Z}} %integers
\newcommand{\CC}{\mathds{C}} %complex numbers
\newcommand{\QQ}{\mathds{Q}} % rational numbers
\newcommand{\perm}{{\cal P}} %permutations
\newcommand{\transp}{\mathfrak{T}} %transpositions

\newcommand{\EE}{\mathds{E}} %expectation
\newcommand{\PP}{\mathds{P}} % proba
\newcommand{\OO}{\mathcal{O}} % grand O pour complexité
\newcommand{\ind}{\mathds{1}} % indicatrice




\DeclareMathOperator*{\diag}{\mbox{diag}}
\DeclareMathOperator*{\tr}{\mbox{tr}}
\DeclareMathOperator*{\card}{\mbox{card}}
\DeclareMathOperator*{\cov}{\mbox{cov}}
\DeclareMathOperator*{\sign}{\mbox{sign}}
\DeclareMathOperator*{\var}{\mbox{var}}
%\DeclareMathOperator*{\st}{\mbox{s.t.}}
\DeclareMathOperator*{\rank}{\mbox{rank}}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\moyenne}{average}

\DeclareMathOperator*{\Ber}{Ber}
\DeclareMathOperator*{\Beta}{Beta}
\newcommand{\Norm}{\mathcal{N}}
\DeclareMathOperator*{\sigmoid}{sigmoid}
\DeclareMathOperator*{\logit}{logit}

\DeclareMathOperator{\KL}{kl}


\newcommand{\indep}{\perp \!\!\! \perp}
%\newcommand{\defeq}{\stackrel{def}{=}}
\newcommand{\defeq}{:=}


\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
